Dynamics-Informed Action Learning for Goal-Conditioned Latent Planning

Latent world models enable visual control by planning action sequences in compact representation spaces, but a gap remains between how latent dynamics are learned and how they are used for planning. First, teacher-forced training does not expose the dynamics model to the recursively predicted latent states encountered during planning. Second, sampling-based planners typically initialize action search from goal-agnostic proposals, without exploiting the action-conditioned dynamics learned by the world model. We introduce Dynamics-Informed Action Learning (DIAL) to bridge these two gaps. During training, rollout alignment exposes the forward model to its own autoregressive latent predictions, while multi-step inverse supervision trains a lightweight inverse dynamics head to infer actions from latent-state transitions. We further apply the inverse head to model-generated transitions with its parameters held fixed, encouraging predicted rollouts to retain action-relevant information. At test time, DIAL autoregressively couples the inverse and forward dynamics to construct a dynamics-informed action sequence toward the goal, which initializes the mean of the Cross-Entropy Method (CEM) proposal distribution. The subsequent CEM search then refines this initialization using the standard sampling and updating procedure. Experiments across four visual control benchmarks demonstrate that DIAL outperforms existing latent world models and planning baselines in both standard and long-horizon scenarios.

==> submission/preamble.tex <==
%% This file contains a number of tweaks that are typically applied to the main document.
%% They are not enabled by default, but can be enabled by uncommenting the relevant lines.

%%
%% Inline annotations; for predefined colors, refer to "dvipsnames" in the xcolor package:
%% https://tinyurl.com/overleaf-colors
%%
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
%%
%% disable for camera ready / submission by uncommenting these lines  
%%
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}

%%
%% work harder in optimizing text layout. Typically shrinks text by 1/6 of page, enable
%% it at the very end of the writing process, when you are just above the page limit
%%
% \usepackage{microtype}

%%
%% fine-tune paragraph spacing
%%
% \renewcommand{\paragraph}[1]{\vspace{.5em}\noindent\textbf{#1.}}

%%
%% globally adjusts space between figure and caption
%%
% \setlength{\abovecaptionskip}{.5em}


%%
%% Allows "the use of \paper to refer to the project name"
%% with automatic management of space at the end of the word
%%
% \usepackage{xspace}
% \newcommand{\paper}{ProjectName\xspace}

%%
%% Commonly used math definitions
%%
% \DeclareMathOperator*{\argmin}{arg\,min}
% \DeclareMathOperator*{\argmax}{arg\,max}

%%
%% Tigthen underline
%%
% \usepackage{soul}
% \setuldepth{foobar}

==> submission/sec/0_abstract.tex <==
\begin{abstract}
Latent world models enable visual control by planning action sequences in compact representation spaces, but a gap remains between how latent dynamics are learned and how they are used for planning. First, teacher-forced training does not expose the dynamics model to the recursively predicted latent states encountered during planning. Second, sampling-based planners typically initialize action search from goal-agnostic proposals, without exploiting the action-conditioned dynamics learned by the world model. We introduce Dynamics-Informed Action Learning (DIAL) to bridge these two gaps. During training, rollout alignment exposes the forward model to its own autoregressive latent predictions, while multi-step inverse supervision trains a lightweight inverse dynamics head to infer actions from latent-state transitions. We further apply the inverse head to model-generated transitions with its parameters held fixed, encouraging predicted rollouts to retain action-relevant information. At test time, DIAL autoregressively couples the inverse and forward dynamics to construct a dynamics-informed action sequence toward the goal, which initializes the mean of the Cross-Entropy Method (CEM) proposal distribution. The subsequent CEM search then refines this initialization using the standard sampling and updating procedure. Experiments across four visual control benchmarks demonstrate that DIAL outperforms existing latent world models and planning baselines in both standard and long-horizon scenarios.
\end{abstract}

==> submission/sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

World models enable agents to predict the consequences of their actions before execution~\cite{ha2018recurrent,hafner2019learning,hafner2019dream}, allowing them to learn from imagined rollouts rather than environment interactions. This paradigm has demonstrated strong performance across diverse control settings, with recent world-model agents achieving broad task coverage and performance surpassing human levels~\cite{hafner2023mastering,hafner2025training}. In visual planning, latent world models bypass pixel-level reconstruction and operate directly in a compact latent space~\cite{maes2026leworldmodel}. During training, forward dynamics models learn how actions transform the current latent state into a future state. At planning time, goal-conditioned control generates candidate action sequences and selects those whose predicted outcomes best match the goal~\cite{sun2026intact}. However, this forward model
defines a one-way, action-conditioned mapping from actions to state transitions: it predicts the resulting state given an action, but does not directly infer which action would induce a desired latent-state transition. This asymmetry creates a gap between learned dynamics and planning.

\begin{figure*}[t]
\centering
\includegraphics[width=\linewidth]{figs/fig1.pdf}
\vspace{-8mm}
\caption{\textbf{DIAL aligns latent dynamics learning with goal-directed planning.}
(a) During training, teacher forcing performs one-step prediction from observed latent states.
(b) At planning time, autoregressive rollouts can accumulate prediction drift, while generic action proposals lack goal-directed initialization.
(c) DIAL addresses both gaps by training on model-generated rollouts and using learned inverse dynamics to construct a dynamics-informed CEM proposal.}
\label{fig:gap}
\vspace{-4mm}
\end{figure*}

This asymmetry appears in two complementary ways. First, there is an inconsistency in the state inputs received by the model during the training and planning phases. During training, each prediction relies on latent states derived from encoded observation frames. Conversely, during planning, the model must autoregressively feed its own predictions into subsequent steps, causing errors to accumulate during the rollout process~\cite{li2026predictive}. Consequently, accurate single-step prediction does not necessarily translate into reliable multi-step planning. Second, existing planning methods fail to fully leverage the action-conditioned dynamics learned by the world model when initializing the action search. Planners typically initialize candidate action sequences based on generic uniform or Gaussian distributions~\cite{de2005tutorial,sun2026intact}, without using this learned information to identify promising regions of the action space toward the goal. As a result, under limited search budgets or large goal offsets, such uninformed initialization forces early iterations to explore irrelevant regions of the action space, reducing search efficiency.

Existing approaches address these challenges mainly from the modeling and trajectory-evaluation perspectives. On the modeling side, methods such as DINO-WM~\cite{zhou2024dino}, PLDM~\cite{sobal2022joint,sobal2025stress}, and LeWM~\cite{maes2026leworldmodel} improve latent representations and dynamics modeling. On the trajectory-evaluation side, methods such as RC-aux~\cite{li2026predictive} and TRM~\cite{li2026beyond} improve candidate evaluation. These approaches, however, do not directly connect learned action-conditioned dynamics to the initialization of goal-conditioned action search. As illustrated in Fig.~\ref{fig:gap}, autoregressive prediction and action-search initialization therefore remain two separate aspects of the planning pipeline.

To this end, we propose \textbf{D}ynamics-\textbf{I}nformed \textbf{A}ction \textbf{L}earning (\textbf{DIAL}) for latent world models. DIAL connects latent dynamics learning with autoregressive planning and uses learned inverse dynamics to inform the initialization of action search. During training, rollout alignment exposes the forward model to its own predicted latent states, while multi-step inverse supervision trains a lightweight inverse dynamics head to recover actions from latent-state transitions. We further apply the inverse head to model-generated transitions with the forward model held fixed, encouraging rollouts to preserve action-relevant information. During planning, the inverse head infers an action toward the goal from the current predicted latent state, and the forward model predicts the resulting latent state for the next step. The resulting action sequence initializes only the mean of the Cross-Entropy Method (CEM) proposal distribution, while the subsequent sampling and proposal-refitting procedure remains unchanged. DIAL therefore transfers action-conditioned information learned during world-model training into goal-directed search without introducing an additional planning stage or increasing the search budget.



We instantiate DIAL on LeWorldModel (LeWM), a compact reconstruction-free JEPA world model for goal-conditioned planning from pixels~\cite{maes2026leworldmodel}. DIAL preserves the original LeWM backbone and CEM planning procedure, allowing us to isolate the effects of rollout-aligned training and dynamics-informed action initialization. We evaluate DIAL on the original LeWM task family under matched training and planning protocols, including different planning horizons, search budgets, and ablation settings. DIAL consistently improves goal-reaching performance, with particularly pronounced gains under limited search budgets and long-horizon goals. These results demonstrate the benefit of combining rollout-aligned latent dynamics with dynamics-informed action initialization for efficient latent planning. Our contributions can be summarized as:

\begin{enumerate}[leftmargin=*,itemsep=2pt]

\item We propose DIAL, a dynamics-informed framework that connects latent dynamics learning with goal-conditioned planning by using learned inverse dynamics to construct initial CEM proposal.

\item We introduce rollout alignment and multi-step inverse supervision to improve autoregressive dynamics and preserve action-relevant information in model-generated latent transitions.

\item We provide controlled empirical evaluation across multiple goal offsets, search budgets, and training ablations, demonstrating consistent improvements in goal-reaching performance, particularly under limited search budgets and long-horizon planning.

\end{enumerate}


==> submission/sec/2_formatting.tex <==
\section{Related Work}
\label{sec:formatting}


\paragraph{World models for representation.}
World models aim to learn predictive models of environment dynamics from data, enabling agents to reason about future states through imagined rollouts. Early approaches rely on generative models that explicitly model future observations, such as IRIS~\cite{micheli2022transformers}, DIAMOND~\cite{alonso2024diffusion}, and DreamerV4~\cite{hafner2025training}. More recently, Joint-Embedding Predictive Architectures (JEPAs) have emerged as a reconstruction-free alternative, learning predictive dynamics directly in a compact latent space without explicit pixel reconstruction. Within action-conditioned latent world modeling, JEPA-based methods differ in how representations are learned. Methods based on frozen pretrained encoders, such as DINO-WM~\cite{zhou2024dino}, constrain the learned state space through pre-trained visual representations. End-to-end approaches such as PLDM~\cite{sobal2022joint,sobal2025stress}, while capable of jointly learning representations and dynamic information from raw observation data, may face training instability issues. LeWM~\cite{maes2026leworldmodel} addresses this challenge with a stable end-to-end framework that combines latent prediction with representation regularization. Our method is based on the end-to-end JEPA framework and investigates how to leverage the learned dynamic model to improve planning.

\paragraph{Candidate evaluation.}
Beyond improving learned representations and dynamics models, another line of work improves planning by refining the objective used to evaluate candidate trajectories. Fast-LeWM~\cite{gao2026fast} introduces a self-consistency score during candidate selection to filter out dynamical hallucinations, while RC-aux~\cite{li2026predictive} and TRM~\cite{li2026beyond} augment the terminal cost with reachability-aware metrics or temporal distance constraints. These approaches primarily improve the evaluation and ranking of generated candidates, while leaving the  proposal distribution unchanged. Consequently, when the search budget is limited or the task requires substantial exploration, the quality of generated candidate set may become a bottleneck that cannot be resolved solely through improved candidate evaluation.

\paragraph{Inverse dynamics and action priors.}

Learned inverse dynamics and action priors have also been explored for visual planning. GC-IDM~\cite{nguyen2026latent}, for example, uses inverse dynamics to directly generate goal-conditioned actions, making planning dependent on the accuracy of the learned action predictor. PRISM~\cite{wang2026prism} learns a goal-conditioned Gaussian prior separately from a frozen world model, leaving the action prior decoupled from the learned dynamics. INTACT~\cite{sun2026intact} incorporates learned intent-to-action mappings into CEM-based~\cite{rubinstein2004cross} planning, primarily using the learned mapping for direct action generation or local search verification. In contrast, DIAL jointly learns inverse dynamics with the latent world model and uses the resulting dynamics-informed action sequence to initialize the CEM proposal mean, while retaining CEM for subsequent candidate sampling and refinement.

==> submission/sec/3_finalcopy.tex <==

\section{Preliminaries}
\label{sec:prelim}

\paragraph{Latent world model.}
Following LeWM~\cite{maes2026leworldmodel}, we consider a reconstruction-free
latent world model consisting of a visual encoder
$E_\phi:\mathcal{O}\rightarrow\mathbb{R}^D$ and an action-conditioned latent
dynamics model $F_\theta$. The encoder maps observations to latent states:
\begin{equation}
z_t = E_\phi(o_t).
\end{equation}
The dynamics model predicts the next latent state from a temporal context of latent states and actions:
\begin{equation}
\hat z_{t+1}
=
F_\theta
\!\left(
z_{t-h+1:t},
a_{t-h+1:t}
\right),
\end{equation}
where $h$ denotes the context length and $a_t$ is the current action used to predict $\hat z_{t+1}$. Following the reconstruction-free formulation of LeWM, the model is trained to predict future latent states from observed trajectories together with an anti-collapse regularizer. At planning time, the learned dynamics model is applied autoregressively to predict the consequences of candidate action sequences.

\paragraph{Goal-conditioned planning.}
We consider finite-horizon goal-conditioned control from visual observations. At time $t$, the agent observes $o_t$ and is given a goal observation $o_g$, with corresponding latent states $z_t$ and $z_g$. Given the current latent context and goal latent, planning seeks an action sequence whose predicted terminal latent is closest to the goal:
\begin{equation}
\begin{aligned}
a_{t:t+H-1}^{*}
\in
\arg\min_{a_{t:t+H-1}}
d\!\left(
\tilde z_{t+H},
z_g
\right),
\\
\tilde z_{t+H}
=
F_\theta^{(H)}
\!\left(
z_{t-h+1:t},
a_{t-h+1:t+H-1}
\right),
\end{aligned}
\end{equation}
where $d(\cdot,\cdot)$ denotes the latent goal-matching cost and
$F_\theta^{(H)}$ denotes the autoregressive $H$-step rollout of
$F_\theta$. The historical actions $a_{t-h+1:t-1}$ are fixed context, while the future actions $a_{t:t+H-1}$ are optimization variables. Planning is typically implemented using sampling-based Model Predictive Control methods, such as the Cross-Entropy Method (CEM)~\cite{rubinstein2004cross}. CEM samples candidate action sequences from a Gaussian proposal distribution, evaluates their terminal latent costs, selects the top $N_{\mathrm{e}}$ elite sequences, and refits the proposal distribution using these elites. This process is repeated for a fixed number of iterations, after which the resulting action sequence is executed in a receding-horizon manner.

\section{Method}
\label{sec:method}

\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{figs/overview.pdf}
    \vspace{-4mm}
\caption{Overview of DIAL. \textbf{(1) Rollout alignment} trains the latent dynamics predictor $F_\theta$ on autoregressively generated latent contexts to reduce the mismatch between training and planning. \textbf{(2) Multi-step inverse supervision} trains the inverse-dynamics head $G_\psi$ on observed latent state pairs and uses a frozen inverse head $G_{\bar\psi}$ to encourage model-generated states to preserve action-relevant information. \textbf{(3) Dynamics-informed planning} autoregressively couples $G_\psi$ and $F_\theta$ to generate a goal-directed action sequence, which initializes only the mean of the CEM proposal.}
    \vspace{-4mm}
    \label{fig:overview}
\end{figure*}

\subsection{Overview}
\label{sec:method-overview}


We propose Dynamics-Informed Action Learning (DIAL) for latent world models, a framework that aligns latent dynamics learning with autoregressive planning and leverages learned inverse dynamics to initialize action search. As illustrated in Fig.~\ref{fig:overview}, DIAL comprises a visual encoder $E_\phi$, an action-conditioned latent predictor $F_\theta$, and a lightweight inverse dynamics head $G_\psi$. The encoder maps observations to $D$-dimensional latent states, while the predictor $F_\theta$ forecasts future latent states based on the current latent state and action context. The proposed inverse dynamics head $G_\psi$ is responsible for estimating the action connecting a pair of latent states.

Building on the base world-model objective, DIAL introduces three complementary training terms. First, rollout alignment trains $F_\theta$ on autoregressively generated latent contexts, reducing the mismatch between teacher-forced training and planning-time rollouts. Second, multi-step inverse supervision trains $G_\psi$ to recover actions from observed latent state pairs. Third, inverse supervision on predicted states applies a frozen copy of the inverse head to model-generated latent pairs, encouraging autoregressive rollouts to preserve action-relevant information. At planning time, DIAL uses $G_\psi$ and $F_\theta$ autoregressively to construct a goal-directed action sequence. Starting from the current latent state, $G_\psi$ estimates an action toward the goal from the current latent state and goal latent, and $F_\theta$ advances the latent state under the predicted action. The resulting sequence initializes only the mean of the CEM proposal distribution, while CEM retains its standard sampling, evaluation, elite selection, proposal refitting, and search budget.

\subsection{Rollout-Aligned Latent Training}
\label{sec:method-train}


\paragraph{Rollout alignment.}
The base prediction objective trains $F_\theta$ with teacher forcing, where each prediction is conditioned on latent states encoded from observed frames. During planning, however, $F_\theta$ is applied autoregressively, so its own predictions become inputs to subsequent steps. To align these two input regimes, we train $F_\theta$ over an autoregressive rollout of depth $L$. Starting from the observed latent context $\tilde z_{t-h+1:t}=z_{t-h+1:t}$, we generate an autoregressive rollout by feeding each predicted latent state back into the predictor. Specifically, the $j$-th predicted state is obtained as:
\begin{equation}
\begin{aligned}
\tilde z_{t+j}
=
F_\theta\!\left(
\tilde z_{t+j-h:t+j-1},
a_{t+j-h:t+j-1}
\right),
\\
j=1,\ldots,L,
\label{eq:ra-rollout}
\end{aligned}
\end{equation}

The first prediction is therefore conditioned entirely on observed latents, while subsequent input windows progressively replace observed states with model predictions. For $j>h$, the predictor is conditioned entirely on model-generated latents. We then minimize the rollout alignment loss as:
\begin{equation}
\mathcal{L}_{\mathrm{RA}}
=
\frac{1}{L}
\sum_{j=1}^{L}
\left\|
\tilde z_{t+j}
-
\mathrm{sg}[z_{t+j}]
\right\|_2^2,
\label{eq:ra-loss}
\end{equation}
where $\mathrm{sg}[\cdot]$ denotes stop-gradient. It is applied only to the target latents, while gradients propagate through complete autoregressive recursion. Thus, $\mathcal{L}_{\mathrm{RA}}$ directly trains $F_\theta$ on model-generated inputs encountered during planning.


\paragraph{Multi-step inverse supervision.}
Rollout alignment improves the reliability of autoregressive states, but does
not explicitly require these states to preserve information about the actions
that caused them. We therefore introduce a lightweight inverse dynamics head
$G_\psi$ to recover the initiating action from a latent-state transition. For
an ordered transition from $z_t$ to $z_{t+k}$, we predict
\begin{equation}
\hat a_t = G_\psi(z_t,z_{t+k}),
\qquad
k=1,\ldots,K_{\mathrm{obs}},
\end{equation}
where the supervision target is always the first action $a_t$. Thus, for
$k>1$, the head recovers the action initiating the transition rather than the
complete intervening action sequence. We train $G_\psi$ on latent-state pairs encoded from observed
trajectories:
\begin{equation}
\mathcal{L}_{\mathrm{obs}}
=
\sum_{k=1}^{K_{\mathrm{obs}}}
\omega_k
\left\|
G_\psi(z_t,z_{t+k})-a_t
\right\|_2^2,
\label{eq:inv-observed}
\end{equation}
where $\omega_k\propto K_{\mathrm{obs}}-k+1$ and
$\sum_k\omega_k=1$. This objective trains the inverse mapping while
encouraging the shared latent representation to retain information about the initiating action. 

We further impose the same recoverability constraint on autoregressively
predicted states. Let $\tilde z_{t+k}$ denote a state generated by the
rollout in Eq.~(\ref{eq:ra-rollout}). We reuse $G_\psi$ on these model-generated
pairs while holding its parameters fixed:
\begin{equation}
\mathcal{L}_{\mathrm{roll}}
=
\frac{1}{K_{\mathrm{roll}}}
\sum_{k=1}^{K_{\mathrm{roll}}}
\left\|
G_\psi\!\left(
\mathrm{sg}[z_t],
\tilde z_{t+k}
\right)-a_t
\right\|_2^2.
\label{eq:inv-rollout}
\end{equation}

During this loss, the parameters of $G_\psi$ are held fixed, so gradients flow through its latent inputs and the autoregressive rollout rather than through the inverse mapping itself. The anchor latent is also detached to prevent this loss from directly updating the first input of $G_\psi$. Consequently, $\mathcal{L}_{\mathrm{obs}}$ learns action recovery from observed transitions, while $\mathcal{L}_{\mathrm{roll}}$ encourages model-generated states to preserve the same action-relevant information.


\paragraph{Overall training objective.}
In addition to the objectives above, we retain the reconstruction-free latent prediction objective of LeWM~\cite{maes2026leworldmodel}:
\begin{equation}
\mathcal{L}_{\mathrm{pred}}
=
\left\|
F_\theta\!\left(
z_{t-\ell+1:t},
a_{t-\ell+1:t}
\right)
-
z_{t+1}
\right\|_2^2.
\label{eq:base-pred}
\end{equation}

The predictor accepts variable-length contexts, and this objective is additionally averaged over all valid context lengths $1\leq\ell\leq h$ rather than supervising only the longest one. Following LeWM, we additionally employ the Sketch Isotropic Gaussian Regularizer (SIGReg) to prevent representation collapse:
\begin{equation}
\mathcal{L}_{\mathrm{WM}}
=
\mathcal{L}_{\mathrm{pred}}
+
\lambda_{\mathrm{sig}}\mathcal{L}_{\mathrm{SIG}}.
\label{eq:base-wm}
\end{equation}

Combining this objective with the DIAL-specific terms yields the full training objective:
\begin{equation}
\mathcal{L}_{\mathrm{DIAL}}
=
\mathcal{L}_{\mathrm{WM}}
+
\beta_{\mathrm{RA}}\mathcal{L}_{\mathrm{RA}}
+
\beta_{\mathrm{obs}}\mathcal{L}_{\mathrm{obs}}
+
\beta_{\mathrm{roll}}\mathcal{L}_{\mathrm{roll}},
\label{eq:method-objective}
\end{equation}
where $\beta_{\mathrm{RA}}$, $\beta_{\mathrm{obs}}$, and $\beta_{\mathrm{roll}}$ control the weights of the three DIAL-specific training terms.

\subsection{Dynamics-Informed Planning}
\label{sec:method-inference}

Standard CEM initializes its proposal with a goal-agnostic Gaussian distribution \(q^{(0)}=\mathcal{N}(\mathbf{0},\Sigma_0)\). At planning time, DIAL uses the learned inverse dynamics head to construct a dynamics-informed proposal sequence. Starting from the current latent state \(\tilde z_t = z_t\), the inverse head recursively predicts an action conditioned on the current predicted state and the goal latent, and the forward model advances the latent state under the predicted action:
\begin{equation}
\begin{aligned}
\mu_{t+i}
&=
G_\psi\!\left(\tilde z_{t+i},z_g\right), \\
\tilde z_{t+i+1}
&=
F_\theta\!\left(\tilde z_{t+i},\mu_{t+i}\right),
\qquad i=0,\ldots,H-1.
\end{aligned}
\label{eq:isp-seed}
\end{equation}

For notational simplicity, Eq.~(\ref{eq:isp-seed}) writes \(F_\theta\) with a single state and action, while in practice the predictor retains the most recent \(h\) latent states and actions, following the same convention as during training. Each action is therefore inferred from the latest predicted latent state, producing a goal-conditioned proposal sequence \(\mu_{t:t+H-1}\). Because \(z_g\) may lie beyond the temporal offsets used to train \(G_\psi\), this sequence is not assumed to be an accurate open-loop plan. This sequence is used only to initialize the mean of the CEM proposal:
\begin{equation}
q^{(0)}
=
\mathcal{N}\!\left(\mu_{t:t+H-1},\Sigma_0\right),
\label{eq:isp-proposal}
\end{equation}
where the initial covariance \(\Sigma_0\) remains unchanged. CEM then proceeds with its standard sampling, model rollout, elite selection, and proposal refitting steps. The inverse-decoded sequence only biases the initial search distribution and is never executed directly. Subsequent CEM iterations can therefore correct errors in the initialization.


\section{Experiments}
\label{sec:experiments}

\subsection{Experimental Setup}
\label{sec:exp-setup}

\paragraph{Environments and datasets.}
We follow the evaluation protocol of LeWM~\cite{maes2026leworldmodel} and use the same offline datasets, observation preprocessing, and goal-conditioned planning setup. The environments include TwoRoom~\cite{sobal2025stress}, PushT~\cite{zhou2024dino}, Reacher~\cite{tassa2018deepmind}, and Cube~\cite{park2025ogbench}. Each episode provides an initial observation and a goal image. We report success rate as the primary metric. We use a standard goal offset of 25 steps and additionally introduce an offset-50 setting to evaluate planning over a substantially larger temporal distance. Within each evaluation setting, all methods use the same interaction and evaluation protocol.


\begin{table*}[t]
  \centering
  \small
  \caption{\textbf{Success rates (\%) at the standard 25-step and long-horizon 50-step goal offsets.} Offset-25 results are quoted from the corresponding papers unless otherwise noted. Offset-50 results are evaluated using a unified harness with identical episodes (\(n=50\)) and the same CEM candidate budget across methods. Bold and underline indicate the best and second-best results.}

  \label{tab:combined}
  \resizebox{\textwidth}{!}{%
  \begin{tabular}{l rrrrr rrrrr}
  \toprule
  \multirow{2}{*}{Method} & \multicolumn{5}{c}{Offset 25} & \multicolumn{5}{c}{Offset 50} \\
  \cmidrule(lr){2-6} \cmidrule(lr){7-11}
   & PushT & Cube & Reacher & TwoRoom & Macro & PushT & Cube & Reacher & TwoRoom & Macro \\
  \midrule
  PLDM~\cite{sobal2022joint,sobal2025stress} & 78.0 & 65.0 & 78.0 & 97.0 & 79.5 & 20.0 & 46.0 & 66.0 & 78.0 & 52.5 \\
  DINO-WM~\cite{zhou2024dino} & 74.0 & 86.0 & 79.0 & \textbf{100.0} & 84.8 & 14.0 & 46.0 & 20.0 & \underline{94.0} & 43.5 \\
  LeWM~\cite{maes2026leworldmodel} & \underline{96.0} & 74.0 & 86.0 & 87.0 & 85.8 & 60.0 & 64.0 & 72.0 & 56.0 & 63.0 \\
  RC-aux~\cite{li2026predictive} & 90.8 & 76.0 & 87.2 & \underline{98.0} & 88.0 & \textbf{64.0} & 54.0 & 82.0 & 54.0 & 63.5 \\
  Fast-LeWM~\cite{gao2026fast} & \underline{96.0} & 80.0 & \underline{88.0} & \underline{98.0} & 90.5 & 46.0 & 58.0 & 80.0 & 50.0 & 58.5 \\
  Qantara~\cite{rakhimov2026qantara} & 90.1 & 93.7 & 80.9 & \textbf{100.0} & 91.2 & 40.0 & \underline{68.0} & 78.0 & 84.0 & 67.5 \\
  Fast-LeWM-SC~\cite{gao2026fast} & \textbf{98.0} & 82.0 & \textbf{90.0} & \underline{98.0} & 92.0 & 50.0 & 62.0 & 78.0 & 50.0 & 60.0 \\
  INTACT (Pure CEM)~\cite{sun2026intact} & 88.4 & 68.4 & 83.7 & 82.9 & 80.9 & 54.0 & 46.0 & 72.0 & 38.0 & 52.5 \\
  INTACT (Actor CEM)~\cite{sun2026intact} & 93.6 & \textbf{96.9} & 86.6 & \underline{98.0} & \underline{93.8} & \underline{62.0} & 48.0 & \underline{86.0} & \textbf{96.0} & \underline{73.0} \\
  \midrule
  \textbf{Ours} & \textbf{98.0} & \underline{96.0} & \textbf{90.0} & \textbf{100.0} & \textbf{96.0} & \underline{62.0} & \textbf{70.0} & \textbf{88.0} & 92.0 & \textbf{78.0} \\
  \bottomrule
  \end{tabular}%
  }
\end{table*}


\paragraph{Planning protocol.}

Following prior work~\cite{maes2026leworldmodel,gao2026fast,li2026predictive}, we use an action block size of 5 and a planning horizon of $H=5$, so each plan spans 25 primitive environment steps. An offset of 25 can therefore be addressed within a single plan, whereas an offset of 50 requires replanning while keeping the per-plan horizon unchanged. Importantly, the long-horizon setting does not increase the CEM search budget or planning horizon. The dynamics-informed sequence is generated once to initialize the CEM proposal mean and does not introduce an additional CEM iteration or candidate rollout. Unless otherwise stated, all methods use the same CEM sampling budget, update rule, and replanning schedule within each evaluation setting.



\paragraph{Baselines.} 
We compare DIAL against prior methods that modify different components of the same goal-conditioned latent planning pipeline. Specifically, PLDM~\cite{sobal2022joint,sobal2025stress}, DINO-WM~\cite{zhou2024dino}, LeWM~\cite{maes2026leworldmodel}, Fast-LeWM~\cite{gao2026fast}, and Qantara~\cite{rakhimov2026qantara} modify the learned representations or the forward dynamics. RC-aux~\cite{li2026predictive} modifies the candidate re-scoring mechanism. INTACT~\cite{sun2026intact} replaces the action proposal distribution with learned action mappings or priors. Among these, LeWM is the closest point of comparison because it shares the same backbone architecture and planning protocol. Where official reports are available, baseline results are cited directly from the original papers. For settings not reported in the original publications, we evaluate methods using officially released checkpoints or retrain them using publicly available implementations, adhering strictly to the standardized evaluation protocol for each benchmark.

\begin{figure*}[t]

\centering

\includegraphics[width=\linewidth]{figs/quantitative.pdf}
\vspace{-8mm}
\caption{\textbf{Visualization of planning trajectories on Cube and PushT.} Compared with LeWM and INTACT, DIAL maintains object interaction and makes greater progress toward the goal, while other methods either lose object interaction or terminate far from target.}
\label{fig:qualitative}
\end{figure*}

\vspace{-8mm}
\subsection{Main Results}
\label{sec:exp-main}


\paragraph{Comparison at the standard 25-step offset.} The left part of Table~\ref{tab:combined} summarizes performance at the standard 25-step offset. DIAL achieves the highest macro success rate of \(96.0\%\). Compared with prior-free LeWM~\cite{maes2026leworldmodel}, DIAL improves the macro score by \(10.2\) points, with particularly large gains of \(22.0\) and \(13.0\) points on Cube~\cite{park2025ogbench} and TwoRoom~\cite{sobal2025stress}, respectively. Compared with Fast-LeWM~\cite{gao2026fast} and RC-aux~\cite{li2026predictive}, which improve candidate evaluation while retaining prior-free proposal initialization, DIAL further improves the macro score by \(5.5\) and \(8.0\) points, respectively. Compared with INTACT~\cite{sun2026intact}, DIAL exceeds its pure CEM and actor CEM variants by \(15.1\) and \(2.2\) points, respectively. The former uses a generic Gaussian proposal, while the latter introduces a separately learned actor for action initialization. DIAL derives its initialization directly from the jointly trained forward and inverse dynamics, without introducing a separate policy training stage.

\begin{figure*}[t]
\centering
\includegraphics[width=\linewidth]{figs/fig_wrong_goal.pdf}
\vspace{-8mm}
\caption{\textbf{Effect of goal consistency in proposal initialization.} Success rates (\%) for uninitialized, mismatched-goal, and matched-goal proposals across environments and goal offsets under the constrained search budget (\(30\times10\), \(n=50\) episodes per setting).}
\vspace{-4mm}
\label{fig:wrong-goal}
\end{figure*}

\paragraph{Comparison at the 50-step long-horizon offset.} We further evaluate long-horizon planning by doubling the goal offset from \(25\) to \(50\) steps while keeping the evaluation and planning protocols unchanged, as shown in the right part of Table~\ref{tab:combined}. DIAL achieves the highest macro success rate of \(78.0\%\), outperforming Qantara~\cite{rakhimov2026qantara} and LeWM~\cite{maes2026leworldmodel} by \(10.5\) and \(15.0\) points, respectively. The largest gain appears on TwoRoom, where DIAL improves over LeWM by \(36.0\) points. On Cube~\cite{park2025ogbench}, DIAL also exceeds the INTACT actor CEM variant~\cite{sun2026intact} by \(22.0\) points. In contrast, the benefit of improving candidate evaluation alone is limited at this longer horizon. For example, Fast-LeWM-SC~\cite{gao2026fast} improves over Fast-LeWM by only \(1.5\) points. These results indicate that as the temporal distance to the goal increases, providing CEM with a goal-conditioned initial proposal becomes increasingly important for effective search under a fixed planning budget.

\paragraph{Qualitative visualization.}

We provide a qualitative comparison of LeWM~\cite{maes2026leworldmodel}, INTACT~\cite{sun2026intact}, and DIAL in Fig.~\ref{fig:qualitative}. The figure shows representative long-horizon rollouts on Cube~\cite{park2025ogbench} (left) and PushT~\cite{zhou2024dino} (right) under the 50-step goal-offset setting. For each task, the first column shows the initial observation, the intermediate columns show the predicted rollout, and the final column shows the goal observation. LeWM and INTACT either lose effective object interaction or make insufficient progress toward the goal, resulting in rollouts that terminate far from the target. In contrast, DIAL maintains object interaction and makes greater progress toward the goal, consistent with its improved long-horizon performance in Table~\ref{tab:combined}.

\begin{figure*}[t]
\centering
\includegraphics[width=0.99\linewidth]{figs/fig_seeding_effect.pdf}
\vspace{-6mm}
\caption{\textbf{Dynamics-informed initialization under constrained budgets.} Success rates (\%) across environments for uninitialized and dynamics-informed proposals under different goal offsets and search budgets. Full and low budgets correspond to \(300\times30\) and \(30\times10\) candidate rollouts.}
\vspace{-4mm}
\label{fig:seeding-effect}
\end{figure*}

\begin{table*}[t]
\caption{\textbf{Loss ablation at the 25-step goal offset under unseeded CEM.} Each variant is trained from scratch with identical architecture and optimization schedule, and evaluated with the full \(300\times30\) budget. Success rates (\%) are reported for different combinations of training objectives.}
\vspace{-2mm}
\label{tab:ladder}
\centering
\small
\setlength{\tabcolsep}{7pt}
\begin{tabular}{ccccccccc}
\toprule
\(\mathcal{L}_{\mathrm{WM}}\) & \(\mathcal{L}_{\mathrm{RA}}\) & \(\mathcal{L}_{\mathrm{obs}}\) & \(\mathcal{L}_{\mathrm{roll}}\) & PushT & Cube & Reacher & TwoRoom & Macro \\
\midrule
\checkmark &  &  &  & \textbf{96.0} & 72.0 & 80.0 & 84.0 & 83.0 \\
\checkmark & \checkmark &  &  & 94.0 & 70.0 & 88.0 & 82.0 & 83.5 \\
\checkmark &  & \checkmark &  & 90.0 & 80.0 & 90.0 & 80.0 & 85.0 \\
\checkmark & \checkmark & \checkmark &  & 94.0 & \textbf{84.0} & 82.0 & \textbf{86.0} & 86.5 \\
\checkmark & \checkmark & \checkmark & \checkmark & \textbf{96.0} & \textbf{84.0} & \textbf{92.0} & \textbf{86.0} & \textbf{89.5} \\
\bottomrule
\end{tabular}
\vspace{-4mm}
\end{table*}


\subsection{Ablation Study}
\label{sec:ablation}

\paragraph{Effect of goal consistency in proposal initialization.}
To determine whether the benefit of DIAL comes from goal-conditioned initialization rather than simply shifting the proposal distribution away from the default prior, we replace the target latent with one from a different episode while keeping the inverse dynamics module and CEM procedure unchanged. We evaluate this control under the constrained \(30\times10\) search budget. As shown in Fig.~\ref{fig:wrong-goal}, correctly matched goal proposals consistently outperform mismatched proposals across all eight environment and offset settings, with an average gap of \(21.5\) percentage points. In most settings, mismatched proposals provide little or no improvement over uninitialized CEM and can even degrade performance. These results indicate that the benefit of proposal initialization depends on its consistency with the target goal, rather than simply on shifting the proposal mean away from the default prior. The target latent therefore provides essential goal-specific information for constructing an informative initial proposal for CEM.






\paragraph{Dynamics-informed initialization under constrained budgets.}

We evaluate dynamics-informed proposal initialization across search budgets and goal offsets (Fig.~\ref{fig:seeding-effect}). At the 25-step offset, initialization improves mean success by \(13.5\) percentage points under the low budget (\(30\times10\)), compared with \(3.5\) points under the full budget (\(300\times30\)), indicating that its benefit is more pronounced when CEM has fewer opportunities to recover through exploration. The effect grows substantially at the 50-step offset with the planning horizon fixed at \(H=5\), where the mean gains increase to \(27.0\) and \(16.0\) points under the low and full budgets, respectively. In particular, TwoRoom improves from \(22\%\) to \(80\%\) under the low budget. These results indicate that dynamics-informed initialization becomes increasingly valuable when the search budget is constrained or the goal is temporally distant.




\paragraph{Loss ablation for model training.}
To assess the contribution of each training objective, Table~\ref{tab:ladder} reports a controlled ablation at the 25-step goal offset. Starting from the teacher-forced baseline (\(\mathcal{L}_{\mathrm{WM}}\)), adding rollout alignment (\(\mathcal{L}_{\mathrm{RA}}\)) provides only a marginal improvement in macro success, from \(83.0\%\) to \(83.5\%\). In contrast, multi-step inverse supervision (\(\mathcal{L}_{\mathrm{obs}}\)) increases macro success to \(85.0\%\), including an \(8.0\)-point gain on Cube. Combining the two objectives further raises macro success to \(86.5\%\). However, \(\mathcal{L}_{\mathrm{obs}}\) enforces action recoverability only on ground-truth transitions and does not directly constrain model-generated rollouts. \(\mathcal{L}_{\mathrm{roll}}\) addresses this limitation by applying the learned inverse head to autoregressively predicted latent pairs, encouraging model-generated transitions to preserve action-relevant information. Adding \(\mathcal{L}_{\mathrm{roll}}\) yields the highest macro success of \(89.5\%\), with the best or tied-best performance on all four tasks: \(96.0\%\) on PushT, \(84.0\%\) on Cube, \(92.0\%\) on Reacher, and \(86.0\%\) on TwoRoom. The results show that preserving action recoverability on both ground-truth transitions and model-generated rollouts is important for effective planning.



\section{Conclusion}

We present Dynamics-Informed Action Learning (DIAL), a framework that connects latent dynamics learning with goal-conditioned planning through rollout-aligned training and learned inverse dynamics. DIAL trains the latent dynamics model on autoregressive rollouts while learning an inverse dynamics head to preserve action-relevant information in both observed and model-generated transitions. At planning time, the learned inverse and forward dynamics are coupled to construct a dynamics-informed action sequence that initializes the mean of the CEM proposal, while the subsequent search procedure remains unchanged. Across four visual planning benchmarks, DIAL improves goal-reaching performance at both standard \(25\)-step and extended \(50\)-step goal offsets, with particularly large gains under constrained search budgets. These results demonstrate that action-conditioned information learned during latent dynamics training can directly guide goal-conditioned search, improving planning without altering the CEM.
